Effective Communication of Scientific Results

Communication is essential for the advancement of Science. Technology advances and the proliferation of personal devices have changed the ways in which people communicate in all aspects of life. Scientific communication has also been profoundly affected by such changes, and thus it is important to reflect on effective ways to communicate scientific results to scientists that are flooded with information. This article advocates for receiver-oriented communication in Science, discusses how effective oral presentations should be prepared and delivered, provides advice on the thought process that can lead to scientific papers that communicate effectively, discusses suitable methodology to produce experimental data that is relevant and offers advice on how to present such data in ways that lead to the formulation of correct claims that are supported by the data.

==> sections/presentations.tex <==
\section{Oral Presentations}

A good process to create an effective presentation starts with a reflection of what should be said, which is the story to be told, and what are the messages that the audience should take away at the end of the presentation. My recommendation is to use a story-telling approach and to imagine that one is not creating a lecture, but rather that one is creating a movie. In the process of creating a movie, there is a story-board stage where the creator lays out the way the story will be told and the illustrations that are needed for each part of the story. Creation of presentation materials should only start after this initial story-board stage. Imagining the whole presentation before preparing the first slide will help to focus in the illustrations and text that make sense. Often, I will at this point create a presentation with all the transition slides. A transition slide contains only a few words and serves as signpost for the presenter and for the audience that the conversation will switch to a new topic or a new aspect of the discussion.

\subsection{Text vs Illustrations in Slides}

All too often slides in lectures and presentations contain large amount of text. The issue is that the cognitive center that are required for reading the text in the same that is needed to comprehend the speech during the presentation. Thus, such slides only create a distraction to the listener and hinder comprehension~\cite{}. This style of slides are often used as speaker notes and are there only to remind the presenter about the sequence of the presentation 
